An Efficient Doubly-Robust Test for the Kernel Treatment Effect

The average treatment effect, which is the difference in expectation of the counterfactuals, is probably the most popular target effect in causal inference with binary treatments. However, treatments may have effects beyond the mean, for instance decreasing or increasing the variance. We propose a new kernel-based test for distributional effects of the treatment. It is, to the best of our knowledge, the first kernel-based, doubly-robust test with provably valid type-I error. Furthermore, our proposed algorithm is computationally efficient, avoiding the use of permutations.

==> spare.tex <==
On the other hand, kernel-based approaches are widely used for distributional tasks, as kernel mean embeddings \citep{muandet2017kernel} can be used for distribution representation. In this context, \citet{gretton2012kernel} proposed the Maximum Mean Discrepancy (MMD) for conducting two-sample tests. \citet{luedtke2019omnibus} extended the work for testing equality in distribution for unknown functions. Alike algorithms such as the Hilbert Schmidt Independence Criterium \citep{gretton2007kernel} have also seen extensive use.

The framework can be generalized in a straightforward manner for discrete $A$; we refer the reader to \citet{kennedy2017non} for the complexities of continuous treatments.

Extensive literature has focused in conditional mean embeddings given their nice asymptotic properties \citep{li2022optimal} under certain assumptions. In experimental settings, the $O(\frac{1}{\sqrt{n}})$ rates are already inferred by the well-specified propensity scores, so highly flexible mean embedding regressors may be used and still achieve such rates.

\begin{definition}[Kernel Mean Embedding (KME)]
Let $\mathcal{P}$ be the set of all probability measures on a measurable space $(\mathcal{X}, \mathcal{B}_\mathcal{X})$, and $k: \mathcal{X} \times \mathcal{X}$ a reproducing kernel with associated RKHS $\mathcal{H}$ such that $\sup_{x \in \mathcal{X}} k(x,x) < \infty$. The kernel mean embedding (KME) of $\mathbb{P} \in \mathcal{P}$ with respect to $k$ is defined as the following Bochner integral
$$\mu^{k}: \mathcal{P} \to \mathcal{H}, \quad \mathbb{P} \to \mu^k_\mathbb{P}:= \int k(\cdot, x) d\mathbb{P}(x).$$
\end{definition}

It can be shown \citep{gretton2012kernel} that 
\begin{align}  \label{eq:mmd}
    \text{MMD}^2(\mathbb{P}, \mathbb{Q}) = \langle \mu_\mathbb{P} - \mu_\mathbb{Q}, \mu_\mathbb{P} - \mu_\mathbb{Q} \rangle_\mathcal{H} = || \mu_\mathbb{P} - \mu_\mathbb{Q} ||_\mathcal{H}^2.
\end{align}
